Putting Data at the Centre of Offline Multi-Agent Reinforcement Learning

Offline multi-agent reinforcement learning (MARL) is an exciting direction of research that uses static datasets to find optimal control policies for multi-agent systems. Though the field is by definition data-driven, efforts have thus far neglected data in their drive to achieve state-of-the-art results. We first substantiate this claim by surveying the literature, showing how the majority of works generate their own datasets without consistent methodology and provide sparse information about the characteristics of these datasets. We then show why neglecting the nature of the data is problematic, through salient examples of how tightly algorithmic performance is coupled to the dataset used, necessitating a common foundation for experiments in the field. In response, we take a big step towards improving data usage and data awareness in offline MARL, with three key contributions: (1) a clear guideline for generating novel datasets; (2) a standardisation of over 80 existing datasets, hosted in a publicly available repository, using a consistent storage format and easy-to-use API; and (3) a suite of analysis tools that allow us to understand these datasets better, aiding further development.

==> _sections-old/1-introduction.tex <==
\section{Introduction}



 RL algorithms typically require extensive online interactions with an environment to be able to learn robust policies \citep{yu2018towards}. This limits the extent to which previously-recorded experience may be leveraged for RL applications, forcing practitioners to instead rely heavily on optimised environment simulators that are able to run quickly and in parallel on modern compute hardware. 

In a simulation, it is not atypical to be able to generate hundreds of years of operating behaviour of a specific system \citep{openai2019dota5, Vinyals2019alphastar}.
However, achieving this level of online data generation throughput in real-world systems, where a realistic simulator is not readily available, can be challenging or near impossible.
More recently, the field of offline RL has offered a solution to this challenge by bridging the gap between RL and supervised learning. In offline RL, the aim is to develop algorithms that are able to leverage large existing datasets of sequential decision-making to learn optimal control strategies that can be deployed online~\citep{levine2020offline}. 
Many researchers believe that offline RL could help unlock the full potential of RL when applied to the real world, where success has been limited~\citep{dulac2021challenges}.

Although the field of offline RL has experienced a surge in research interest in recent years \citep{prudencio2023offlinerl}, the focus on offline approaches specific to the multi-agent setting has remained relatively neglected, despite the fact that many real-world problems are naturally formulated as multi-agent systems (e.g. traffic management \citep{zhang2019cityflow}, a fleet of ride-sharing vehicles \citep{sykora2020marvin}, a network of trains \citep{mohanty2020flatland} or electricity grid management \citep{khattar2022citylearn}). Moreover, systems that require multiple agents (programmed and/or human) to execute coordinated strategies to perform optimally, arguably have a higher barrier to entry when it comes to creating bespoke simulators to model their online operating behaviour. 

Offline RL research in the single agent setting has benefited greatly from publicly available datasets such as D4RL~\citep{fu2020d4rl} and RL Unplugged~\citep{gulcehre2020rl}. Without such offerings in the multi-agent setting to help standardise research efforts and evaluation, it remains challenging to gauge the state of the field and reproduce results from previous work. Ultimately, to develop new ideas that drive the field forward, standardised datasets and baselines are required.

In this paper, we present OG-MARL, a rich set of datasets specifically curated for cooperative offline MARL. We generated diverse datasets on a range of popular cooperative MARL environments. For each environment, we provide different types of behaviour resulting in \textit{Good}, \textit{Medium} and \textit{Poor} datasets as well as \textit{Replay} datasets (a mixture of the previous three). We developed and applied a quality assurance methodology to validate our datasets to ensure that they contain a diverse spread of experiences. Together with our datasets, we provide initial baseline results using state-of-the-art offline MARL algorithms. 

The OG-MARL code and datasets are publicly available through our anonymised website.\footnote{\url{https://sites.google.com/view/og-marl}} Additionally, we invite the community to contribute their own datasets to the growing repository on OG-MARL and use our website as a platform for storing and distributing datasets for the benefit of the research community. We hope the lessons contained in our methodology for generating and validating datasets help future researchers to produce high-quality offline MARL datasets and help drive progress. 



==> _sections-old/10-checklist.tex <==
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See \autoref{sec:limitations}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See \autoref{sec:limitations}.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Our datasets and code are open-sourced.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{All of the training details are in \autoref{sec:baselines} and the hyperparameter details are in \autoref{sec:appendix_baselines}.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{See \autoref{fig:perf_profiles}.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See \autoref{sec:appendix_baselines}.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerNA{}
  \item Did you mention the license of the assets?
    \answerYes{See our datasheet in \autoref{sec:appendix_datasheet} and licence in \autoref{sec:licence}.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}{See our datasheet in \autoref{sec:appendix_datasheet}.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{See our datasheet in \autoref{sec:appendix_datasheet}.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{See our datasheet in \autoref{sec:appendix_datasheet}.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> _sections-old/2-prelims.tex <==
\section{Preliminaries}

\begin{figure}
    \centering
    \includegraphics[width=0.6\textwidth]{figures/og-marl-crop.pdf}
    \caption{An illustration of offline MARL. Behaviour policies collect experiences and store them in an offline dataset. New policies are trained from the offline data without any online environment interactions. At the end of training, the policies are deployed in the environment.}
    \label{fig:og-marl}
\end{figure}

\textbf{Multi-Agent Reinforcement Learning.} There are three main formulations of MARL tasks: competitive, cooperative and mixed. The focus of this work is on the cooperative setting. Cooperative MARL can be formulated as a \textit{decentralised partially observable Markov decision process} (Dec-POMDP)~\citep{bernstein2002decpomdp}. A Dec-POMDP consists of a tuple $\mathcal{M}=(\mathcal{N}, \mathcal{S}, \{\mathcal{A}^i\}, \{\mathcal{O}^i\}$, $P$, $E$, $\rho_0$, $r$, $\gamma)$, where $\mathcal{N}\equiv \{1,\dots,n\}$ is the set of $n$ agents in the system and $s\in \mathcal{S}$ describes the full state of the system. The initial state distribution is given by $\rho_0$. Each agent $i\in \mathcal{N}$ receives only partial information from the environment in the form of a local observation $o^i_t$, given according to an emission function $E(o_t|s_t, i)$. At each timestep $t$, each agent chooses an action $a^i_t\in\mathcal{A}^i$ to form a joint action $\mathbf{a}_t\in\mathcal{A} \equiv \prod^N_i \mathcal{A}^i$. Due to partial observability, each agent typically maintains an observation history $o^i_{0:t}=(o^i_0,\dots, o^i_t)$, or implicit memory, on which it conditions its policy $\mu^i(a_{t}^i|o^i_{0:t})$, when choosing an action. The environment then transitions to a new state in response to the joint action selected in the current state, according to the state transition function $P(s_{t+1}|s_t, \mathbf{a}_t)$ and provides a shared scalar reward to each agent according to a reward function $r(s,a):\mathcal{S}\times \mathcal{A} \rightarrow \mathbb{R}$. We define an agent's return as its discounted cumulative rewards over the $T$ episode timesteps, $G=\sum_{t=0}^T \gamma^t r_t$, where $\gamma \in (0, 1]$ is the discount factor. The goal of MARL in a Dec-POMDP is to find a joint policy $(\pi^1, \dots, \pi^n) \equiv \mathbf{\pi}$ such that the return of each agent $i$, following $\pi^i$, is maximised with respect to the other agents’ policies, $\pi^{-i} \equiv (\pi \backslash \pi^i)$. That is, we aim to find $\pi$ such that
$\forall i: \pi^i \in {\arg\max}_{\hat{\pi}^i} \mathbb{E}\left[G \mid \hat{\pi}^i, \pi^{-i}\right]$

\textbf{Offline Reinforcement Learning.} An offline RL algorithm is trained on a static, previously collected dataset $\mathcal{D}_\beta$  of transitions $(o_t, a_t, r_t, o_{t+1})$ from some (potentially unknown) behaviour policy $\pi_\beta$, without any further online interactions. There are several well-known challenges in the offline RL setting which have been explored, predominantly in the single-agent literature. The primary issues are related to different manifestations of data distribution mismatch between the offline data and the induced online data. \cite{levine2020offline} provide a detailed survey of the problems and solutions in offline RL.

\textbf{Offline Multi-Agent Reinforcement Learning.} In the multi-agent setting, offline MARL algorithms are designed to learn an optimal \textit{joint} policy $(\pi^1, \dots, \pi^n) \equiv \mathbf{\pi}$, from a static dataset $\mathcal{D}_\beta^\mathcal{N}$ of previously collected multi-agent transitions $(\{o^1_t,\dots,o^n_t\},\{a^1_t,\dots,a^n_t\},\{r_t^1,\dots,r_t^n\},\{o^1_{t+1},\dots,o^n_{t+1}\})$, generated by a set of interacting behaviour policies $(\pi^1_\beta, \dots,~\pi^n_\beta) \equiv \mathbf{\pi_\beta}$.

==> _sections-old/3-related.tex <==
\section{Related Work}

\textbf{Datasets. }
In the single-agent RL setting, D4RL~\citep{fu2020d4rl} and RL~Unplugged~\citep{gulcehre2020rl} have been important contributions, providing a comprehensive set of offline datasets for benchmarking offline RL algorithms. 
While not originally included, D4RL was later extended by~\cite{lu2022challenges} to incorporate datasets with pixel-based observations, which they highlight as a notable deficiency of other datasets. The ease of access to high-quality datasets provided by D4RL and RL Unplugged has enabled the field of offline RL to make rapid progress over the past years \citep{kostrikov2021offline, ghasemipour2022so, nakamoto2023cal}. However, these repositories lack datasets for MARL, which we believe, alongside additional technical difficulties such as large joint action spaces~\citep{yang2021believe}, has resulted in slower progress in the field.

\textbf{Offline Multi-Agent Reinforcement Learning. }
To date, there has been a limited number of papers published on cooperative offline MARL, resulting in benchmarks, datasets and algorithms that do not adhere to any unified standard, making comparisons between works difficult. In brief,
\citet{zhang2021finitesample} carried out an in-depth theoretical analysis of finite-sample offline MARL. \cite{jiang2021marldecentralised} proposed a decentralised multi-agent version of the popular offline RL algorithm BCQ \citep{fujimoto2019bcq} and evaluated it on their own datasets of a multi-agent version of MuJoCo (MAMuJoCo) \citep{peng2021facmac}. \citet{yang2021believe} highlighted how extrapolation error accumulates rapidly in the number of agents and propose a new method they call \textit{Implicit Constraint Q-Learning} (ICQ) to address this. The authors evaluate their method on their own datasets collected using the popular \textit{StarCraft Mulit-Agent Challenge} (SMAC) \citep{samvelyan2019smac}. \citet{pan2022plan} showed that \textit{Conservative Q-Learning} (CQL) \citep{kumar2020cql}, a very successful offline RL method, does not transfer well to the multi-agent setting since the multi-agent policy gradients are prone to uncoordinated local optima. To overcome this, the authors proposed a zeroth-order optimization method to better optimize the conservative value functions, and evaluate their method on their own datasets of a handful of SMAC scenarios, the two agent HalfCheetah scenario from MAMuJoCo and some simple Multi Particle Environments (MPE) \citep{lowe2017maddpg}. \citet{meng2021madt} propose a \textit{multi-agent decision transformer} (MADT) architecture, which builds on the \textit{decision transformer} (DT) \citep{chen2021decision}, and demonstrated how it can be used for offline pre-training and online fine-tuning in MARL by evaluating their method on their own SMAC datasets. \cite{barde2023modelbased} explored a model-based approach for offline MARL and evaluated their method on MAMuJoCo. 

\textbf{Datasets and baselines for Offline MARL. } In all of the aforementioned works, the authors generate their own datasets for their experiments and provide only a limited amount of information about the composition of their datasets (e.g. spread of episode returns and/or visualisations of the behaviour policy). Furthermore, each paper proposes a novel algorithm and typically compares their proposal to a set of baselines specifically implemented for their work. The lack of commonly shared benchmark datasets and baselines among previous papers has made it difficult to compare the relative strengths and weaknesses of these contributions and is one of the key motivations for our work.

Finally, we note works that have already made use of the pre-release version of OG-MARL. \cite{formanek2023reduce} investigated selective ``reincarnation'' in the multi-agent setting and \cite{zhu2023madiff} explored using diffusion models to learn policies in offline MARL. Both these works made use of OG-MARL datasets for their experiments, which allows for easier reproducibility and more sound comparison with future work using OG-MARL.

==> _sections-old/4-properties.tex <==
\section{Task Properties}
In order to design an offline MARL benchmark which is maximally useful to the community, we carefully considered the properties that the environments and datasets in our benchmark should satisfy. A major drawback in most prior work has been the limited diversity in the tasks that the algorithms were evaluated on. \cite{meng2021madt} for example only evaluated their algorithm on SMAC datasets and \cite{jiang2021marldecentralised} only evaluated on MAMuJoCo datasets. This makes it difficult to draw strong conclusions about the generalisability of offline MARL algorithms. Moreover, these environments fail to test the algorithms along dimensions which may be important for real-world applications. In this section, we outline the properties we believe are important for evaluating offline MARL algorithms.

\textbf{Centralised and Independent Training. } The environments supported in OG-MARL are designed to test algorithms that use decentralised execution, i.e.\ at execution time, agents need to choose actions based on their local observation histories only. However, during training, centralisation (i.e.\ sharing information between agents) is permissible, although not required. \textit{Centralised training with decentralised execution} (CTDE) \citep{kraemer2016multi} is one of the most popular MARL paradigms and is well-suited for many real-world applications. Being able to test both centralised and independent training algorithms is important because it has been shown that neither paradigm is consistently better than the other \citep{lyu2021contrasting}. As such, both types of algorithms can be evaluated using OG-MARL datasets and we also provide baselines for both centralised and independent training.

\textbf{Different types of Behaviour Policies.} We generated datasets with several different types of behaviour policies including policies trained using online MARL with fully independent learners (e.g. independent DQN and independent TD3), as well as CTDE algorithms (e.g. QMIX and MATD3).  Furthermore, some datasets generated with CTDE algorithms used a state-based critic while others used a joint-observation critic. It was important for us to consider both of these critic setups as they are known to result in qualitatively different policies \citep{lyu2022deeper}. More specific details of which algorithms were used to generate which datasets can be found in \autoref{tab:all_environments} in the appendix.

\textbf{Partial Information.} It is common for agents to receive only local information about their environment, especially in real-world systems that rely on decentralised components. Thus, some of the environments in OG-MARL test an algorithm's ability to leverage agents' \textit{memory} in order to choose optimal actions based only on partial information from local observations. This is in contrast to settings such as MAMuJoCo where prior methods \citep{jiang2021marldecentralised, pan2022plan} achieved reasonable results without instilling agents with any form of memory.

\textbf{Different Observation Modalities.} In the real world, agent observations come in many different forms. For example, observations may be in the form of a feature vector or a matrix representing a pixel-based visual observation. \cite{lu2022challenges} highlighted that prior single-agent offline RL datasets failed to test algorithms on high-dimensional pixel-based observations. OG-MARL tests algorithms on a diverse set of observation modalities, including feature vectors and pixel matrices of different sizes.

\textbf{Continuous and Discrete Action Spaces.} The actions an agent is expected to take can be either discrete or continuous across a diverse range of applications. Moreover, continuous action spaces can often be more challenging for offline MARL algorithms as the larger action spaces make them more prone to extrapolation errors, due to out-of-distribution actions \cite{}. OG-MARL supports a range of environments with both discrete and continuous actions.

\textbf{Homogeneous and Heterogeneous Agents.} Real-world systems can either be homogeneous or heterogeneous in terms of the types of agents that comprise the system. In a homogeneous system, it may be significantly simpler to train a single policy and copy it to all agents in the system. On the other hand, in a heterogenous system, where agents may have significantly different roles and responsibilities, this approach is unlikely to succeed. OG-MARL provides datasets from environments that represent both homogeneous and heterogeneous systems.

\textbf{Number of Agents.} Practical MARL systems may have a large number of agents. Most prior works to date have evaluated their algorithms on environments with typically fewer than 8 agents \citep{pan2022plan, yang2021believe, jiang2021marldecentralised}. In OG-MARL, we provide datasets with between 2 and 27 agents, to better evaluate \textit{large-scale} offline MARL (see \autoref{tab:all_environments}). 

\textbf{Sparse Rewards.} Sparse rewards are challenging in the single-agent setting, but in the multi-agent setting, it can be even more challenging due to the multi-agent credit assignment problem \citep{zhou2020learning}. Prior works focused exclusively on dense reward settings \citep{pan2022plan,yang2021believe}. To overcome this, OG-MARL also provides datasets with sparse rewards. 

\textbf{Team and Individual Rewards.} Some environments have team rewards while others can have an additional local reward component. Team rewards exacerbate the multi-agent credit assignment problem, and having a local reward component can help mitigate this. However, local rewards may result in sub-optimality, where agents behave too greedily with respect to their local reward and as a result jeopardize achieving the overall team objective. OG-MARL includes tasks to test algorithms along both of these dimensions.

\textbf{Procedurally Generated and Stochastic Environments.} Some popular MARL benchmark environments are known to be highly deterministic \citep{ellis2022smacv2}. This limits the extent to which the generalisation capabilities of algorithms can be evaluated. Procedurally generated environments have proved to be a useful tool for evaluating generalisation in single-agent RL \citep{cobbe2020}. In order to better evaluate generalisation in offline MARL, OG-MARL includes stochastic tasks that make use of procedural generation.

\textbf{Realistic Multi-Agent Domains.} Almost all prior offline MARL works have evaluated their algorithms exclusively on game-like environments such as StarCraft~\citep{yang2021believe} and particle simulators~\citep{pan2022plan}. Although a large subset of open research questions may still be readily investigated in such simulated environments, we argue that in order for offline MARL to become more practically relevant, benchmarks in the research community should begin to closer reflect real-world problems of interest. Therefore, in addition to common game-like benchmark environments, OG-MARL also supports environments which simulate more real-world like problems including energy management and control~\citep{vazquezcanteli2020citylearn,wang2021voltage}. While there remains a large gap between these environments and truly real-world settings, it is a step in the right direction to keep pushing the field forward and enable useful contributions in the development of new algorithms and improving our understanding of key difficulties and failure modes.

\textbf{Human Behaviour Policies.} The current standard practice in the offline MARL literature is to use policies trained using RL as the behaviour policies for offline MARL datasets. However, for real-world applications, behaviour policies are likely to be non-RL policies such as human operators or hand-crafted controllers. In order to encourage the offline MARL community to move beyond RL behaviour policies, we provide a dataset of humans playing the \textit{Knights, Archers and Zombies} game from PettingZoo. It is our hope that this contribution will catalyse more research on offline MARL from human-generated data.

\textbf{Competitive Scenarios.} Competitive offline MARL is an under researched area with only a handful of existing works in the field \citep{cui2022provably}. Moreover, all of the existing works have almost exclusively focused on tabular two-player zero-sum Markov games \citep{cui2021minimax,zhong2022pessimistic}. In order to encourage the offline MARL research community to make advances in the competitive offline setting, we provide a dataset on the popular competitive \textit{MPE} environment, \textit{Simple Adversary}. Furthermore, the offline data recorder in OG-MARL can readily be used by researchers to generate their own competitive offline datasets on novel environments.

==> _sections-old/5-environments.tex <==
\section{Environments}

\begin{figure}
\centering
    \begin{subfigure}[t]{0.175395\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/environments/smac.png}
        \caption{SMAC}
        \label{fig:smac}
        \centering
        \includegraphics[width=\textwidth]{figures/environments/mamujoco.png}
        \caption{MAMuJoCo}
        \label{fig:mamujoco}
    \end{subfigure}
    \begin{subfigure}[t]{0.175395\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/environments/flatland.png}
        \caption{Flatland}
        \label{fig:flatland}
        \centering
        \includegraphics[width=\textwidth]{figures/environments/city_learn.png}
        \caption{CityLearn}
        \label{fig:citylearn}
    \end{subfigure}
    \begin{subfigure}[t]{0.175395\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/environments/pistonball.png}
        \caption{Pistonball}
        \label{fig:pistonball}
        \centering
        \includegraphics[width=\textwidth]{figures/environments/coop_pong.png}
        \caption{Co-op Pong}
        \label{fig:coop_pong}
    \end{subfigure}
    \begin{subfigure}[t]{0.175395\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/environments/pursuit.png}
        \caption{Pursuit}
        \label{fig:pursuit}
        \centering
        \includegraphics[width=\textwidth]{figures/environments/voltage.png}
        \caption{V. C.} % NOTE (CLAUDE) need shorter name than "Voltage Control"
        \label{fig:voltage}
    \end{subfigure}
    \begin{subfigure}[t]{0.175395\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/environments/kaz.png}
        \caption{KAZ}
        \label{fig:kaz_env}
        \centering
        \includegraphics[width=\textwidth]{figures/environments/mpe.png}
        \caption{MPE}
        \label{fig:mpe}
    \end{subfigure}
\caption{MARL environments for which we provide datasets in OG-MARL.}
    \label{fig:envs}
\end{figure}

\textbf{SMAC v1} \textit{(hetero- and homogeneous agents, local observations)}. SMAC is the most popular cooperative offline MARL environment used in the literature\citep{gorsane2022emarl}. SMAC focuses on the micromanagement challenge in StarCraft 2 where each unit is controlled by an independent agent that must learn to cooperate and coordinate based on local (partial) observations. SMAC played an important role in moving the MARL research community beyond grid-world problems and has also been very popular in the offline MARL literature \citep{yang2021believe, meng2021madt, pan2022plan}. Thus, it was important for OG-MARL to support a range of SMAC scenarios.

\textbf{SMAC v2} \textit{(procedural generation, local observations)}. Recently some deficiencies in SMAC have been brought to light. Most importantly, SMAC is highly deterministic, and agents can therefore learn to \textit{memorise} the best policy by conditioning on the environment timestep only. To address this, SMACv2 \citep{ellis2022smacv2} was recently released and includes non-deterministic scenarios, thus providing a more challenging benchmark for MARL algorithms. In OG-MARL, we publicly release the first set of SMACv2 datasets.

\textbf{MAMuJoCo} \textit{(hetero- and homogeneous agents, continuous actions)}. The MuJoCo environment \citep{todorov2012mujoco} has been an important benchmark that helped drive research in continuous control. More recently, MuJoCo has been adapted for the multi-agent setting by introducing independent agents that control different subsets of the whole MuJoCo robot (MAMuJoCo) \citep{peng2021facmac}. MAMuJoCo is an important benchmark because there are a limited number of continuous action space environments available to the MARL research community. MAMuJoCo has also been widely adopted in the offline MARL literature \citep{jiang2021marldecentralised, pan2022plan}. Thus, in OG-MARL we provide the largest openly available collection of offline datasets on scenarios in MAMuJoCo (\cite{pan2022plan}, for example, only provided a single dataset on 2-Agent HalfCheetah).

\textbf{PettingZoo} \textit{(pixel observations, discrete and continuous actions)}. OpenAI's Gym \citep{brockman2016openai} has been widely used as a benchmark for single agent RL. PettingZoo is a gym-like environment-suite for MARL \citep{terry2021pettingzoo} and provides a diverse collection of environments. In OG-MARL, we provide a general-purpose environment wrapper which can be used to generate new datasets for any PettingZoo environment. Additionally, we provide initial datasets on three PettingZoo environments including \textit{PistonBall}, \textit{Co-op Pong} and \textit{Pursuit}~\citep{gupta2017cooperative}. We chose these environments because they have visual (pixel-based) observations of varying sizes; an important dimension along which prior works have failed to evaluate their algorithms.

\textbf{Flatland} \textit{(real-world problem, procedural generation, sparse local rewards)}. The train scheduling problem is a real-world challenge with significant practical relevance. Flatland~\citep{mohanty2020flatland} is a simplified 2D simulation of the train scheduling problem that is an appealing benchmark for cooperative MARL for several reasons. Firstly, it randomly generates a new train track layout and timetable at the start of each episode, thus testing the generalisation capabilities of MARL algorithms to a greater degree than many other environments. Secondly, Flatland has a very sparse and noisy reward signal, as agents only receive a reward on the final timestep of the episode. Finally, agents have access to a local reward component. These properties make the Flatland environment a novel, challenging and realistic benchmark for offline MARL. 

\textbf{Voltage Control and CityLearn} \textit{(real-world problem, continuous actions)}. Energy management \citep{yu2021energy} is another appealing real-world application for MARL, especially given the large potential efficiency gains and corresponding positive effects on climate change that could be had~\citep{rolnick2022climate}. As such, we provide datasets for two challenging MARL environments related to energy management. Firstly, we provide datasets for the \textit{Active Voltage Control on Power Distribution Networks} environment \citep{wang2021voltage}. Secondly, we provide datasets for the CityLearn environment \citep{vazquezcanteli2020citylearn} where the goal is to develop agents for distributed energy resource management and demand response between a network of buildings with batteries and photovoltaics.

\textbf{Knights, Archers \& Zombies} \textit{(human behaviour policies)}. In \textit{Knights, Archers and Zombies}~\citep{terry2021pettingzoo} (KAZ) zombies walk from the top border of the screen down to the bottom border in unpredictable paths. The agents controlled are a knight and an archer which can each move around and attack the zombies. The game ends when all agents die (collide with a zombie) or a zombie reaches the bottom screen border. We collected experience of several different combinations of human players. The players where given no instruction on how to play the game and had to learn through trial and error. 

\textbf{MPE} \textit{(competitive)}. MPE is a popular suite of multi-agent environments, first introduced by \citep{lowe2017maddpg}. We provide a dataset with baselines on the popular \textit{Simple Adversary} environment \citep{terry2021pettingzoo}.



==> _sections-old/6-datasets.tex <==
\section{Datasets}

To generate the transitions in the datasets, we recorded environment interactions of partially trained online algorithms, as has been common in prior works for both single-agent \citep{gulcehre2020rl} and multi-agent settings \citep{yang2021believe,pan2022plan}. For discrete action environments, we used QMIX~\citep{rashid2018qmix} and independent DQN \cite{} and for continuous action environments, we used independent TD3 \citep{fujimoto2018td3} and MATD3~\citep{lowe2017maddpg, ackermann2019matd3}. Additional details about how each dataset was generated are included in \autoref{section:appendix_datasets}.

\begin{figure}
    \centering
    \begin{subfigure}[]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/violins/27m_vs_30m_all_violin.png}
        \caption{SMAC 27m\_vs\_30m}
        \label{fig:violin_27m_vs_30m}
    \end{subfigure}
    \begin{subfigure}[]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/violins/coop_pong_all_violin.png}
        \caption{PettingZoo Co-op Pong}
        \label{fig:violin_coop_pong}
    \end{subfigure}
    \begin{subfigure}[]{0.32\textwidth}
        \includegraphics[width=\textwidth]{figures/violins/pursuit_all_violin.png}
        \caption{PettingZoo Pursuit}
        \label{fig:violin_pursuit}
    \end{subfigure}
    \caption{Violin plots of the probability distribution of episode returns for selected datasets in OG-MARL. In blue the \texttt{Poor} datasets, in orange the \texttt{Medium} datasets and in green the \texttt{Good} datasets. Wider sections of the violin plot represent a higher probability of sampling a trajectory with a given episode return, while the thinner sections correspond to a lower probability. The violin plots also include the median, interquartile range and min/max episode return for the datasets.}
    \label{fig:violin}
\end{figure}

\textbf{Diverse Data Distributions.} It is well known from the single-agent offline RL literature that the quality of experience in offline datasets can play a large role in the final performance of offline RL algorithms \citep{fu2020d4rl}. In OG-MARL, we include a range of dataset distributions including \texttt{Good}, \texttt{Medium}, \texttt{Poor} and \texttt{Replay} datasets in order to benchmark offline MARL algorithms on a range of different dataset qualities. The dataset types are characterised by the quality of the joint policy that generated the trajectories in the dataset, which is the same approach taken in previous works \citep{meng2021madt, yang2021believe, pan2022plan}. To ensure that all of our datasets have sufficient coverage of the state and action spaces, while also containing minimal repetition i.e.\ not being too narrowly focused around a single strategy, we used 3 independently trained joint policies to generate each dataset, and additionally added a small amount of exploration noise to the policies. The boundaries for the different categories were assigned independently for each environment and were related to the maximum attainable return in the environment. Additional details about how the different datasets were curated can be found in \autoref{section:appendix_datasets}.

\textbf{Statistical characterisation of datasets.} It is common in both the single-agent and multi-agent offline RL literature for researchers to curate offline datasets by unrolling episodes using an RL policy that was trained to a desired \textit{mean} episode return. However, authors seldom report the distribution of episode returns induced by the policy. Reporting only the mean episode return of the behaviour policy can be  misleading~\citep{agarwal2021deep}. To address this, we provide violin plots to visualise the distribution of expected episode returns. A violin plot is a powerful tool for visualising numerical distributions as they visualise the density of the distribution as well as several summary statistics such as  the minimum, maximum and interquartile range of the data. These properties make the violin plot very useful for understanding the distribution of episode returns in the offline datasets, assisting with interpreting offline MARL results. \autoref{fig:violin} provides a sample of the violin plots for different scenarios (the remainder of the plots can be found in the appendix). In each figure, the difference in shape and position of the three violins illustrates the difference in the datasets with respect to the expected episode return. Additionally, we provide a table with the mean and standard deviation of the episode returns for each of the datasets in \autoref{tab:all_datasets}, similar to \cite{meng2021madt}.


==> _sections-old/7-baselines.tex <==
\section{Baselines}\label{sec:baselines}

\begin{table}
\centering
\small
\caption{Results on the \textit{Pursuit} and \textit{Co-op Pong} datasets. The mean episode return with one standard deviation across all seeds is given. In each row the best mean episode return is in bold.}
\vspace{1em}
\begin{tabular}{lclllll}
\textbf{Scenario}        & \textbf{Dataset} & \multicolumn{1}{c}{\textbf{BC}} & \multicolumn{1}{c}{\textbf{QMIX}} & \multicolumn{1}{c}{\textbf{QMIX+BCQ}} & \multicolumn{1}{c}{\textbf{QMIX+CQL}} & \multicolumn{1}{c}{\textbf{MAICQ}} \\ \hline
\multirow{3}{*}{Co-op Pong}    & Good             & 31.2$\pm$3.5                    & 0.6$\pm$3.5                       & 1.9$\pm$1.1                           & \textbf{90.0$\pm$4.7}                 & 75.4$\pm$3.9                       \\
                         & Medium           & 21.6$\pm$4.8                    & 10.6$\pm$17.6                     & 20.3$\pm$12.2                         & 64.9$\pm$15.0                         & \textbf{84.6$\pm$0.9}              \\
                         & Poor             & 1.0$\pm$0.9                     & 14.4$\pm$16.0                     & 30.2$\pm$20.7                         & 52.7$\pm$8.5                          & \textbf{74.8$\pm$7.8}              \\ \hline
\multirow{3}{*}{Pursuit} & Good             & 78.3$\pm$1.8                    & 6.7$\pm$19.0                      & 66.9$\pm$14.0                         & 54.4$\pm$6.3                          & \textbf{92.7$\pm$3.7}              \\
                         & Medium           & 15.0$\pm$1.6                    & -24.4$\pm$20.2                    & 16.6$\pm$10.7                         & 20.6$\pm$10.3                         & \textbf{35.3$\pm$3.0}              \\
                         & Poor             & -18.5$\pm$1.6                   & -43.7$\pm$5.6                     & \textbf{-0.7$\pm$4.0}                 & -19.6$\pm$3.3                         & -4.1$\pm$0.7                       \\ \midrule 
\bottomrule
\end{tabular}
\label{tab:pettingzoo_results}
\end{table}

 In this section, we present the initial baselines that we provide with OG-MARL. This serves two purposes: \textit{i)} to validate the quality of our datasets and \textit{ii)} to enable the community to use these initial results for development and performance comparisons in future work. In the main text, we present results on two PettingZoo environments (\textit{Pursuit} and \textit{Co-op Pong}), since these environments and their corresponding datasets are a novel benchmark for offline MARL. Furthermore, it is the first set of environments with pixel-based observations to be used to evaluate offline MARL algorithms. We include all additional baseline results (including on MPE and KAZ) in \autoref{sec:appendix_baselines}.

 \textbf{Baseline Algorithms.} State-of-the-art algorithms were implemented from seminal offline MARL work. For discrete action environments we implemented \textit{Behaviour Cloning} (BC), QMIX \citep{rashid2018qmix}, QMIX with \textit{Batch Constrained Q-Learning} \citep{fujimoto2019bcq} (QMIX+BCQ), QMIX with \textit{Conservative Q-Learning} \citep{kumar2020cql} (QMIX+CQL) and MAICQ \citep{yang2021believe}. For continuous action environments, Behaviour Cloning (BC), Independent TD3 (ITD3), ITD3 with \textit{Behaviour Cloning} regularisation \citep{fujimoto2021td3bc} (ITD3+BC), ITD3 with \textit{Conservative Q-Learning} (ITD3+CQL) and OMAR \citep{pan2022plan} were implemented. \autoref{sec:appendix_baselines} provides additional implementation details on the baseline algorithms.

 \textbf{Experimental Setup.} On \textit{Pursuit} and \textit{Co-op Pong}, all of the algorithms were trained offline for $50 000$ training steps with a fixed batch size of $32$. At the end of training, we evaluated the performance of the algorithms by unrolling the final joint policy in the environment for $100$ episodes and recording the mean episode return over the episodes. We repeated this procedure for $10$ independent seeds as per the recommendation by \citet{gorsane2022emarl}. We kept the online evaluation budget \citep{kurenkov2022onlineEvalBudget} fixed for all algorithms by only tuning hyper-parameters on \textit{Co-op Pong} and keeping them fixed for \textit{Pursuit}. Controlling for the online evaluation budget is important when comparing offline algorithms because online evaluation may be expensive, slow or dangerous in real-world problems, making online hyper-parameter fine-tuning infeasible. See \autoref{sec:appendix_baselines} for a further discussion on hyper-parameter tuning in OG-MARL.

 \textbf{Results.} In \autoref{tab:pettingzoo_results} we provide the unnormalised mean episode returns for each of the discrete action algorithms on the different datasets for \textit{Pursuit} and \textit{Co-op Pong}. 
 % Results on the other environments and datasets can be found in \autoref{tab:all_discrete_results} and \autoref{tab:all_cont_results}.

\textbf{Aggregated Results.} In addition to the tabulated results we also provide \textit{aggregated} results as per the recommendation by \cite{gorsane2022emarl}. In \autoref{fig:perf_profiles} we plot the performance profiles \citep{agarwal2021deep} of the discrete action algorithms by aggregating across all seeds and the two environments, \textit{Pursuit} and \textit{Co-op Pong}. To facilitate aggregation across environments, where the possible episode returns can be very different, we adopt the normalisation procedure from \citet{fu2020d4rl}. On the \texttt{Good} datasets, we found that MAICQ and QMIX+CQL both outperformed behaviour cloning (BC). QMIX+BCQ did not outperform BC and vanilla QMIX performed very poorly. On the \texttt{Medium} datasets, MAICQ and QMIX+CQL once again performed the best, significantly outperforming BC. QMIX+BCQ marginally outperformed BC and vanilla QMIX failed. Finally, on the \texttt{Poor} datasets, MAICQ, QMIX+CQL and QMIX+BCQ all outperformed BC but MAICQ was the best by some margin. These results on PettingZoo environments, with pixel observations, further substantiate that MAICQ is the current state-of-the-art offline MARL algorithm in discrete action settings. 

\textbf{Reproducibility Statement.} Scripts for easily reproducing all baseline results are provided in our open-sourced code and can be downloaded from the anonymised OG-MARL website.

\begin{figure}
    \begin{subfigure}{0.3\textwidth}
        \includegraphics[width=\textwidth]{figures/baselines/Good_performance_profile.png}
        \caption{Good}
    \end{subfigure}
    \begin{subfigure}{0.3\textwidth}
        \includegraphics[width=\textwidth]{figures/baselines/Medium_performance_profile.png}
        \caption{Medium}
    \end{subfigure}
    \begin{subfigure}{0.3\textwidth}
        \includegraphics[width=\textwidth]{figures/baselines/Poor_performance_profile.png}
        \caption{Poor}
    \end{subfigure}
    \caption{Performance profiles \citep{agarwal2021deep} aggregated across all seeds on \textit{Pursuit} and \textit{Co-op Pong}. Shaded regions show pointwise 95\% confidence bands based on percentile bootstrap with stratified sampling.}
    \label{fig:perf_profiles}
\end{figure}

==> _sections-old/8-conclusions.tex <==
\section{Discussion}

\textbf{Limitations and future work.} \label{sec:limitations} An exciting research direction considers the offline RL problem as a sequence modeling task~\citep{chen2021decision, meng2021madt}, and in future iterations of OG-MARL we aim to incorporate such models as additional baselines. Additionally, some works have explored using diffusion models for offline MARL \citep{li2023conservatism, zhu2023madiff}, which presents another avenue for leveraging OG-MARL in future work.

\textbf{Potential Negative Societal Impacts. } While the potential positive impacts of efficient decentralized controllers powered by offline MARL are promising, it is essential to acknowledge and address the potential negative societal impacts \citep{whittlestone2021societal}. Deploying a model trained using offline MARL in real-world applications requires careful consideration of safety measures \citep{gu2022safety, xu2022constraints}. Practitioners should exercise caution to ensure the implementation of such models is safe and responsible.

\textbf{Conclusion. } In this work, we highlighted the importance of offline MARL as a research direction for applying RL to real-world problems. We specifically focused on the lack of a standard set of benchmark datasets, which currently poses a significant obstacle to measuring meaningful progress across different works. To address this issue, we presented a set of relevant and diverse datasets for offline MARL. We profiled our datasets by visualising the distribution of episode returns in violin plots and tabulated mean and standard deviations. We validated our datasets by providing a set of initial baseline results with state-of-the-art offline MARL algorithms. Finally, we open-sourced all of our software tooling for generating new datasets and provided a website for hosting and sharing datasets. We hope that the research community will adopt and contribute towards OG-MARL as a framework for offline MARL research and that it helps to drive progress in the field.

==> _sections-old/9-acknowledgements.tex <==
% Include in deanonymised version.

% \section*{Acknowledgements}
% We would like to thank Callum Rhys Tilbury for his valuable comments on this work.

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> sections/2-prelims.tex <==
\section{Preliminaries} \label{sec:preliminaries}

\textbf{Multi-Agent Reinforcement Learning.} There are three main formulations of MARL tasks: competitive, cooperative and mixed. The focus of this work is on the cooperative setting. Cooperative MARL can be formulated as a \textit{decentralised, partially observable Markov decision process} (Dec-POMDP)~\citep{bernstein2002decpomdp}. A Dec-POMDP consists of a tuple $\mathcal{M}=(\mathcal{N}, \mathcal{S}, \{\mathcal{A}^i\}, \{\mathcal{O}^i\}$, $P$, $E$, $\rho_0$, $r$, $\gamma)$, where $\mathcal{N}\equiv \{1,\dots,n\}$ is the set of $n$ agents in the system and $s\in \mathcal{S}$ describes the full state of the system. The initial state distribution is given by $\rho_0$. Each agent, $i\in \mathcal{N}$, receives only partial information from the environment in the form of a local observation, $o^i_t$, given according to an emission function $E(o_t|s_t, i)$. At each timestep, $t$, each agent chooses an action, $a^i_t\in\mathcal{A}^i$, to form a joint action, $\mathbf{a}_t\in\mathcal{A} \equiv \prod^N_i \mathcal{A}^i$. Due to partial observability, each agent typically maintains an observation history $o^i_{0:t}=(o^i_0,\dots, o^i_t)$, or implicit memory, on which it conditions its policy $\mu^i(a_{t}^i|o^i_{0:t})$, when choosing an action. The environment then transitions to a new state in response to the joint action selected in the current state, according to the state transition function, $P(s_{t+1}|s_t, \mathbf{a}_t)$, and provides a shared scalar reward to each agent according to a reward function, $r(s,a):\mathcal{S}\times \mathcal{A} \rightarrow \mathbb{R}$. We define an agent's return as its discounted cumulative rewards over the $T$ episode timesteps, $G=\sum_{t=0}^T \gamma^t r_t$, where $\gamma \in (0, 1]$ is the discount factor. The goal of MARL in a Dec-POMDP is to find a joint policy $(\pi^1, \dots, \pi^n) \equiv \mathbf{\pi}$ such that the return of each agent $i$, following $\pi^i$, is maximised with respect to the other agents’ policies, $\pi^{-i} \equiv (\pi \backslash \pi^i)$. That is, we aim to find $\pi$ such that
$\forall i: \pi^i \in {\arg\max}_{\hat{\pi}^i} \mathbb{E}\left[G \mid \hat{\pi}^i, \pi^{-i}\right]$.

\textbf{Offline Reinforcement Learning.} An offline RL algorithm is trained on a static, previously collected dataset $\mathcal{D}_\beta$  of transitions $(o_t, a_t, r_t, o_{t+1})$ from some (potentially unknown) behaviour policy $\pi_\beta$, without any further online interactions. There are several well-known challenges in the offline RL setting which have been explored, predominantly in the single-agent literature. The primary issues are related to different manifestations of data distribution mismatch between the offline data and the induced online data. \citet{levine2020offline} provide a detailed survey of the problems and solutions in offline RL.

\textbf{Offline Multi-Agent Reinforcement Learning.} In the multi-agent setting, offline MARL algorithms are designed to learn an optimal \textit{joint} policy, $(\pi^1, \dots, \pi^n) \equiv \mathbf{\pi}$, from a static dataset $\mathcal{D}_\beta^\mathcal{N}$ of previously collected multi-agent transitions, $$(\{o^1_t,\dots,o^n_t\},\{a^1_t,\dots,a^n_t\},\{r_t^1,\dots,r_t^n\},\{o^1_{t+1},\dots,o^n_{t+1}\}),$$ generated by a set of interacting behaviour policies, $(\pi^1_\beta, \dots,~\pi^n_\beta) \equiv \mathbf{\pi_\beta}$. 

% A depiction of the offline MARL approach is shown in~\Cref{fig:og-marl}.

% \begin{figure}[hbtp]
%     \centering
%     \includegraphics[width=0.8\textwidth]{figures/og-marl-crop.pdf}
%     \caption{An illustration of offline MARL. Behaviour policies collect experiences and store them in an offline dataset. New policies are trained from the offline data without any online environment interactions. At the end of training, the policies are deployed in the environment.}
%     \label{fig:og-marl}
% \end{figure}

==> sections/A-map-to-vault.tex <==
\appendix

\section{Appendix / supplemental material}


\input{tables/map_to_vault}

==> sections/old/old-4-copy.tex <==
\section{Characterising datasets and their effect on offline MARL experiments}\label{sec:control}

Having surveyed the state of the offline MARL field in section \ref{sec:lit-review}, we now present our evidence to support our claim that the field is failing to adequately control for data's impact on their experimental results. The consequence of this is that accurately measuring progress across different works in the field is very challenging. First, in Section \ref{sec:summary-stats}, we set out to demonstrate the significant impact that dataset properties given by simple summary statistics such as the mean and standard deviation of episode returns can have on experimental outcomes. We present our findings in the context of the apparent disregard for the reporting of these properties by works in the field (see table \ref{tab:datasets}). In section \ref{sec:distributions} we attempt to highlight that while summary statistics may be important, they are not necessarily sufficient to properly interpret offline MARL experiments. We use the result to emphasise the utility of visualising the distribution of episode returns in a dataset, a step which is currently widely overlooked by the field. Finally, in section \ref{sec:action-space} we highlight the limits of using the distribution of episode returns as a measure of the diversity of a dataset. Instead, we propose an extension of an idea first proposed by \citet{schweighofer2022dataset} in the single-agent setting called State-Action Coverage (SACo). We extended SACo to the multi-agent setting by computing a decentralised observation-action coverage (DecOACo) score for each agent independently, as well as state and joint-observation coverage scores.


% First, we focus on datasets in their role as control variables. We investigate the following questions: What are the most basic properties to standardise and is the field adhering to that at all? How do these properties affect performance - can they actually change algorithm preferences? If we standardised these properties, would we be able to standardise across different datasets? Are there other properties common to similarly-labelled datasets by which we could justify the standardisation of different datasets?

% Our findings show that a) the field does not standardise basic properties of datasets b) these same properties when varied can produce significantly different performance for the same algorithm c) even if we did standardise these properties, performance of the same algorithm can differ significantly on two different datasets and d) if a set of fully descriptive properties of a dataset exists, it is not clear what that set might be.

% In section \ref{sec:lit-review}, we noted that neither environment version, nor episode return mean nor episode return standard deviation are standardised across the datasets available in the offline MARL field. We now demonstrate that differences in these characteristics of a dataset can significantly affect the results produced using that dataset.

% To demonstrate how dramatic the performance discrepancy can be with even a slight mismatch in environment versioning, we report in \autoref{fig:mamujoco-versions} the performance of MADDPG+CQL trained on several Multi-Agent MuJoCo datasets but in one case the algorithm was evaluated with MuJoCo version 2.0 and another with MuJoCo 2.1. Since the dataset was generated using MuJoCo 2.1, it makes sense that the algorithm performed best when evaluated with the same version. Evaluating under version 2.0 (only one minor release version difference) caused significantly worse final performance. %The second accessibility challenge is that some works do not share download information for their datasets, or share links that are broken. Furthermore, information on how to use the datasets is usually scarce. 

% Others had similar versioning issues online\footnote{\url{https://github.com/ling-pan/OMAR/issues/3}}.

% \begin{figure}[hbtp]
%     \centering
%     \includegraphics[width=0.8\textwidth]{figures/datasets/mamujoco_versions.pdf}
%     \caption{In order to demonstrate that a minor mismatch between dataset and evaluation environment versioning can result in large performance discrepancies, we compared the performance of MADDPG+CQL on MAMuJoCo using Mujoco version 2.0 in one case and MuJoCo version 2.1 in another. The dataset was generated using MuJoCo version 2.1. We aggregated our results across datasets from three scenarios: \texttt{2 Agent HalfCheetah}, \texttt{2 Agent Ant} and \texttt{4 Agent Ant}. We also repeated each experiment across 10 random seeds. To aggregate across scenarios, we first normalised the results.}
%     \label{fig:mamujoco-versions}
% \end{figure}

\subsection{Episode return summary statistics} \label{sec:summary-stats}
In the single-agent offline RL literature, it is very common to use the summary statistics, mean and standard deviation, of the episode, returns to characterise a dataset. Datasets with a higher mean episode return are often given labels such as "Good" or "Expert". Similarly, the standard deviation of episode return is commonly used as a proxy for dataset diversity and datasets with large standard deviations are often labelled "Mixed". Despite being widely reported in the single-agent literature, table \ref{tab:datasets} highlights how commonly offline MARL works fail to report these two statistics. In section \ref{sec:mean} and \ref{sec:std} we test the effect that the mean and standard deviation have on experimental outcomes respectively. We believe these experiments are valuable because at present the field seems to be taking their effects for granted (and is hence commonly omitted in papers).

\subsubsection{Mean} \label{sec:mean}
To test the effect that the mean episode return has on offline MARL experiments we construct datasets with different means on three different SMAC \citep{} scenarios. For each dataset we keep the standard deviation fixed at 2 and the number of episodes fixed to 2000. For both the mean and standard deviation there is a small margin of error (see table \ref{}) since we construct the datasets by sub-sampling episodes from OG-MARL datasets \citep{formanek2023ogmarl}.  We then train two offline MARL algorithms on each dataset respectively and report the final evaluation episode return. We repeat the experiment across 10 random seeds. We then aggregated all results across scenarios, algorithms and seeds using bootstrap confidence intervals \citep{agarwal2021deep,gorsane2022emarl}. 

\begin{figure}[hbtp]
    \centering
    \begin{tabular}{c}
        \begin{subfigure}[p]{0.35\textwidth}
            \centering
            \scriptsize
            \setstretch{1.5}
                \begin{tabular}{c|c}
                & $\mu$ \\\hline
                \dotred & $7\pm0.1$  \\
                \dotgreen & $10\pm0.1$  \\
                \dotorange & $13\pm0.1$  \\
                \dotblue & $16\pm0.1$  \\
                \bottomrule
                \end{tabular}
        \caption{Mean episode return for each class of dataset. Datasets were generated for three SMAC scenarios \texttt{5m\_vs\_6m}, \texttt{3s5z\_vs\_3s6z} and \texttt{2s3z}.}
        \label{fig:mean-matters-means}
        \vspace{1em}
      \end{subfigure}\\
      \end{tabular}
    \hspace{1em}
    \begin{subfigure}[p]{0.55\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/datasets/mean_matters.pdf}
         \caption{Results comparing the final performance of offline MARL algorithms trained on datasets with different mean episode returns. Results are aggregated using bootstrap confidence intervals \citep{agarwal2021deep}. To facilitate aggregation across different scenarios and algorithms, results are first normalised.}
         \label{fig:mean-matters-results}
    \end{subfigure}
      \caption{To demonstrate the effect that the mean episode return of a dataset has on the final performance of an offline MARL algorithm, we generated four datasets with mean episode returns given in \autoref{fig:mean-matters-means}. We then train an offline MARL algorithm for 50k training steps on each of the datasets and compare the final performance of the algorithm across the different datasets. Finally, we repeated the experiment across three different SMAC scenarios, two different algorithms and 10 random seeds. The aggregated results are given in \autoref{fig:mean-matters-results}.}
\label{fig:mean-matters}
\end{figure}

Figure \ref{fig:mean-matters} illustrates that the mean episode return of the dataset is positively correlated with the final performance of the two algorithms we tested. While this may seem obvious, it is clear that without knowing the mean episode return of a dataset used in one paper, it would be very challenging to know how to compare the result to another work that used a different dataset with a different mean. Comparing the final performance of an offline RL algorithm to the mean episode return of the dataset is common practice in the single-agent literature~\citep{gulcehre2020rl, agarwal2019optimistic}, but currently, very few offline MARL researchers are doing it.

\subsubsection{Standard deviation} \label{sec:std}

Arguably one of the most important properties of a dataset in offline RL is experience diversity \citep{agarwal2019optimistic}. In the single-agent setting, it is well-understood that many offline RL algorithms benefit from more diverse datasets~\citep{schweighofer2022dataset}. It is usually beneficial because diverse experience leads to better coverage of the state and action spaces, resulting in fewer out-of-distribution (OOD) actions, which are a known to cause issues when training offline~\citep{fujimoto2019bcq}. However, we believe that the effect of diversity in the offline MARL setting is less well understood and should not be naively taken for granted given the knowledge from the single-agent setting. Work by \citet{pjap} studying two player polynomial games points to there being a more intricate relationship between dataset diversity and final performance in the offline MARL setting than might have been assumed by the community. To test the effect that the standard deviation has on the outcome of an offline MARL experiment in practice, we generate several datasets on SMAC with varying standard deviations, similar to the previous section for the mean. Once again, we repeat the experiment across three scenarios, two algorithms and ten random seeds.

\begin{figure}[hbtp]
    \centering
    \begin{subfigure}[p]{0.47\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/datasets/std_matters_hist.pdf}
         \caption{Histograms of the episode returns of five datasets with differing standard deviations but the same mean are given.}
         \label{fig:std_matters_violins}
    \end{subfigure}
    \hspace{1em}
    \begin{tabular}{c}
        \begin{subfigure}[p]{0.46\textwidth}
            \centering
            \scriptsize
            \setstretch{1.5}
                \begin{tabular}{c|cc}
                 & $\mu$ & $\sigma^2$ \\\hline
                \dotblue & $10\pm0.1$ & $0.5\pm0.02$ \\
                \dotorange & $10\pm0.1$ & $1.0\pm0.1$ \\
                \dotgreen & $10\pm0.1$ & $2.0\pm0.1$ \\
                \dotred & $10\pm0.1$ & $4.0\pm0.1$ \\
                \dotpurple & $10\pm0.1$ & $6.0\pm0.1$ \\
                \bottomrule
                \end{tabular}
        \caption{Dataset mean and standard deviation.}
        \vspace{1em}
      \end{subfigure}\\
    %\noalign{\bigskip}%
      \begin{subfigure}[p]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/datasets/std_matters_results.pdf}
         \caption{The aggregated results across scenarios, algorithms and random seeds are given for each dataset. The median, interquartile mean and mean are all given with bootstrap confidence intervals \citep{agarwal2021deep}.}
         \label{fig:std_matters}
      \end{subfigure}
      \end{tabular}
      \caption{To demonstrate the surprising effect that the standard deviation (std) can have on the performance of an offline MARL experiment we generated 5 datasets that each had the same mean but differing std. We then trained an algorithm on the data and reported the final performance. We repeated the experiment across three different SMAC scenarios, 2 two different algorithms and 10 random seeds. We then aggregated the results as per \cite{gorsane2022emarl}.}
\end{figure}

In \autoref{fig:std_matters}, we see that the performance of the offline MARL algorithms is not optimal with either a very large or a very small standard deviation. Instead, algorithms performed the best when the episode return's standard deviation was somewhere in the middle. This surprising result (from the perspective of a single-agent offline RL researcher) reinforces our argument that papers in offline MARL should report the standard deviation of the episode return in their datasets precisely because our understanding of its effect is not widely understood. Furthermore, it highlights that there is still plenty of research to be done to explore how the quality and diversity of multi-agent data affect the final performance of offline MARL algorithms.

\subsection{Episode return distribution} \label{sec:distributions}

We have shown that varying the basic descriptive properties of datasets can produce varying performance. However, we acknowledge the limitations of these descriptive properties in determining how an algorithm will perform on a given dataset.

In \autoref{fig:mean_std_not_enough} we demonstrate that the performance of offline MARL algorithms may differ even when trained on two datasets that have very similar summary statistics, and identical environment versions. One can see from \autoref{fig:std_and_mean_hist} that while the mean and standard deviation of the datasets are quite similar, their episode return \textit{distributions} are quite distinct, which we argue can have a large impact on the final performance. This highlights that while reporting summary statistics about one's dataset is important, it is not enough to fully describe a dataset. Visualising the dataset distribution is also an essential step, which no one in the multi-agent field is adopting, in contrast to the single-agent field. This is akin to the famous Anscombe's quartet example, where four datasets with identical summary statistics have remarkably different distributions when plotted. We have gone a step further to show that the difference in the dataset composition which may be detected using visualisations have a significant effect on algorithm performance.

\begin{figure}[hbtp]
    \centering
    \begin{subfigure}[p]{0.46\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/datasets/std_and_mean_hist.pdf}
         \caption{Histogram of the episode returns in either dataset.}
         \label{fig:std_and_mean_hist}
    \end{subfigure}
    \hspace{1em}
    \begin{tabular}{c}
    \begin{subfigure}[p]{0.46\textwidth}
         \centering
         \scriptsize
         \setstretch{1.5}
         \begin{tabular}{c|cc}
                 & $\mu$ & $\sigma^2$ \\\hline
                \dotorange & $3688$ & $2885$ \\
                \dotblue & $3665$ & $2866$ \\
                \bottomrule
        \end{tabular}
        \caption{Mean and standard deviation of either dataset.}
        \vspace{1em}
      \end{subfigure}\\
    \begin{subfigure}[p]{0.45\textwidth}
        \centering
         \includegraphics[width=\textwidth]{figures/datasets/std_and_mean_results_halfcheetah.pdf}
         \caption{The aggregated results across ten random seeds for each dataset. The median, interquartile mean and mean are all given with bootstrap confidence intervals \citep{agarwal2021deep}.}
         \label{fig:mean_std_not_enough}
     \end{subfigure}
    \end{tabular}
     \caption{We generated two datasets on 2-Agent Halfcheetah each with very similar episode return means and standard deviations, but distinct data distributions. We then trained MADDPG+CQL on each dataset and reported its final performance after 50,000 training steps. We repeated the experiment over 10 random seeds.}
\end{figure}

\subsection{Multi-agent action coverage} \label{sec:action-space}



For multi-agent offline MARL, dataset diversity has an unpredictable effect on algorithm performance. We showed this in the previous section by varying episode return spread in a dataset and observing that with increasing spread, performance at first increases and then decreases. This is a surprising result because in the single-agent offline RL field it is generally accepted that greater diversity in a dataset is beneficial for algorithm performance.

It is clear that the effect of dataset diversity is not well understood in offline MARL. We further propose that dataset diversity itself is not well understood in offline MARL. Although the most-reported proxy to dataset diversity is episode return standard deviation, it is still just that - a proxy. Following  \citep{schweighofer2022dataset}, we now extend the field's understanding of dataset diversity by considering the counts of unique state-action pairs and observation-action pairs in a dataset. This is a direct measure of diversity within a dataset.

The goal of this extension is two-fold: first, to measure dataset diversity from both a centralised and independent perspective, and second to be able to compare datasets according to their compositions. We first formalise the various coverages we measure, and then we apply our measures to a cross-section of the datasets available in the offline MARL field.

\subsubsection{Defining coverage measures}

We define SACo in the multi-agent setting as though the system is centralised; when we talk about actions in the context of SACo, we mean the joint action. This measure corresponds, as single-agent SACo does, to the coverage of the state-action space of the overall POMDP.

Experience diversity may, however, be viewed in a more nuanced way in the MARL setting. When we consider a decentralised system, the most natural measure of experience diversity for a single agent is the ratio between the number of unique observation-action pairs it experiences and the total number of transitions in the dataset. We call this measure Decentralised Observation-Action Coverage, or DecOACo.

And finally, since we want to interpret DecOACo in the context of decentralisation, we must account for the partial observability of the environment which may also play a role in lowering pair counts. We therefore  measure the ratio of unique joint-observation-joint-action pairs to the total number of transitions in a dataset and call it JOJACo. 

The difference between SACo and JOJACo is a measure of the knowledge gap incurred by partial observability of the environment. The difference between JOJACo and DecOACo is a measure of the partial observability incurred by making a system decentralised. And the difference between SACo and DecOACo is a measure of the total reduction in observability. Note that these measures are not necessarily accessible in online MARL - gaining environment insight before training is an advantage unique to offline MARL.
% so that we differentiate between low DecOACo counts as a result of decentralisation versus as a result of the partial observability of the environment itself.

% \citet{schweighofer2022dataset} propose SACo as a measure of dataset diversity. SACo is defined as the ratio between the number of unique state-action pairs in a dataset and the total number of state-action pairs in that dataset. In the multi-agent setting, SACo is the same as in the single-agent setting, only the action is the joint. 

% A single agent in a multi-agent system may, however, have far fewer unique experiences than the system as a whole.

% From the perspective of one agent, though, there may be far less experience diversity than the count of unique state-action pairs suggests. For each agent, we define the ratio between the count of unique observation-action pairs and the total count of state-joint-action pairs in a dataset 

\subsubsection{Coverage versus episode return spread on a cross-section of the field}

Our cross-section of the datasets available in the field focus on the $5m\_vs\_6m$ task from the popular benchmark environment SMAC. We compare datasets available from \citet{formanek2023ogmarl,cfcql,omiga} on this task first based on their episode return statistics, then based on their coverage measures.

% We take a cross-section of the datasets available in the field by selecting the $5m\_vs\_6m$ task from the popular benchmark environment SMAC. The $5m\_vs\_6m$ task is generally considered a difficult task \citep{madt} and it is covered by all the dataset sources \citep{formanek2023ogmarl,cfcql,omiga} we were able to access. 

% The process required to convert all datasets into as standard a format as possible is described in Appendix. Most importantly, we subsample all datasets uniformly to within an episode of $20~000$ transitions. The purpose of this is to make analysis more tractable, but also to compare dataset composition without needing to account for large differences in dataset sizes. Descriptive characteristics of the subsampled datasets may be found in Appendix, and it can be noted they almost exactly match the reported characteristics of the larger datasets.

\textbf{Diversity in terms of episode return.} As previously discussed, dataset diversity in offline MARL is seldom reported, and when it is, it is in the form of a single standard deviation value for episode return. We have shown that the distribution of episode returns has an effect on algorithm performance on that dataset; following our own suggestions, we visualise all the datasets in our cross-section in Figure \ref{fig:violin_5m_vs_6m}.

\begin{figure}[hbtp]
     \centering
     \includegraphics[scale=0.5]{figures/saco_and_oaco/violin_5m_vs_6m_20000.vlt.pdf}
     \caption{Distributions in the form of a violin plot of episode returns for each subsampled dataset.}
     \label{fig:violin_5m_vs_6m}
\end{figure}

Note the distributions of episode return differ between sources. \citet{formanek2023ogmarl} and \citet{cfcql} generate their own datasets using policies trained by IDRQN and QMIX respectively, while the datasets from \citet{omiga} are subsets from datasets generated by \citet{madt}, the originals of which are no longer accessible. Since datasets from \citet{formanek2023ogmarl} and \citet{cfcql} are rollouts of policies, the episode return distributions of their datasets are allowed to overlap. It is clear, however, that from the generation process employed either by \citet{cfcql} to subsample or by \citep{madt} to generate the original datasets, that the datasets accessed from \citet{cfcql} had explicit limitations on the range of episode returns allowed in each of their datasets.

According to Figure \ref{fig:violin_5m_vs_6m}, and even when comparing episode return means and standard deviations, it may be expected that the datasets "Medium-Replay", "Medium" and "Expert"  from \citet{cfcql} might be easily exchangeable with the datasets "Poor", "Medium" and "Good" from \citet{formanek2023ogmarl}, respectively. Their episode return distributions look similar, and their means and standard deviations follow the same trends with increasing dataset quality.

\textbf{Diversity in terms of coverage}

We plot SJACo, JOJACo and DecOACo for all available datasets. Note that despite having similar-looking distributions, cfcql-medium-replay and OG-MARL Poor are quite differently-composed.

\begin{figure}[hbtp]
    \centering
    \includegraphics[scale=0.5]{figures/saco_and_oaco/OACo_heatmap.png}
    \caption{The counts of unique observation-action pairs and counts of unique state-action pairs for datasets on the 5m vs 6m SMAC task.}
    \label{fig:oaco-placeholder}
\end{figure}

% For datasets from \citet{formanek2023ogmarl}, less than $15\%$ of state-action pairs are repeats of previously-seen pairs. This may be surprising considering the datasets are generated by rolling out a frozen policy, and given that the starting point is deterministic for the version of SMAC used. The "Poor" dataset has fewer unique per-agent observation-action pairs, which can be explained by a more frequent observation of the death state (all observation inputs are 0 and the only available action is 0). However, it is not a general trend that datasets with high episode return mean have more unique pairs, because the "Good" and "Medium" datasets have similar numbers of per-agent unique pairs. Interestingly, the counts in the "Poor" dataset differ significantly between agents, which implies that agents play different roles in the "Poor" datasets. One theory is that agent death is more imbalanced - that is, some agents are positioned to die sooner, and so they experience fewer novel states.

% Datasets from \citet{omiga} subsampled from \citet{madt} have far fewer state-action pair repeats, with the "Good" dataset experiencing less than $5\%$ repeated state-action pairs. There is also a trend where dataset quality increases with fewer state-action pair repeats. This trend is also observed in the per-agent pair counts; the average observation-action pair counts are Good: $20265.4$, Medium: $17839.2$, Poor: $16240.4$.

% Datasets from \citet{cfcql} have considerably lower state-action counts, specifically where replay data is not included. The "Expert" and "Medium" datasets are composed of at least $50\%$ repeated state-action pairs. For each dataset different agents experience similar numbers of unique pairs - role formation cannot be observed in this metric. The "Medium" dataset has agents experiencing on average only around $8000$ unique state-action pairs on dataset of about $25000$ transitions.

% Overall, the death state is a large component of the counts results seen in Figure \ref{fig:oaco-placeholder}. When looking at the counts of unique pairs across dataset sources, trends are not consistent, and counts vary wildly for state-action pairs and per-agent observation-action pairs. This indicates that the performance obtained on datasets from one source is not necessarily comparable to datasets from another source.

% Perhaps an example of how hard it is to access the data?

\subsection{Takeaways}

All of our findings point towards each unique dataset being exactly that - unique. Although we observed some trends in algorithm performance when varying dataset summary statistics, some of those trends were surprising and can absolutely not be assumed to have a simple general form for all dataset-algorithm combinations. We therefore stress that a) assumptions from single-agent offline RL can not be implanted into offline MARL and b) while it is important to test offline algorithms on a variety of datasets, it is not clear what variety means in the offline context, nor which axis of property variation in a dataset will provide adequate coverage of the desired problem space for offline MARL.

 The first steps towards producing adequate coverage of the desired problem space for offline MARL is to specify what exactly the desired problem space is. The fact that this topic has not specifically been covered speaks further to the community's lack of awareness surrounding data, and the fact that a "task" is now a property of a dataset rather than a variable, and the dataset itself might not provide adequate coverage of the task which produced it.

 Which is surprising, since the problem of inadequate coverage is a core issue in offline MARL which needs far more understanding to be solved. Every paper which attempts to address out-of-distribution actions (just cite a bunch here) is dealing with coverage problems.
 
 In Section (ref solns), we propose guidelines for using datasets as control variables, but first in section (ref next section) we take a better look at coverage and the effect of a static dataset on algorithms, and we take explorative steps towards understanding the composition of a multi-agent POMDP dataset, based on the insights we gain from that.

==> sections/old/old-4-standardisation.tex <==
\section{The impact of data in offline MARL}\label{sec:control}

Data is a fundamental component of offline learning, but has not been given the appropriate treatment in much of the literature thus far.  With immense focus on algorithmic innovation instead, the impact of data has been neglected. We argue that this approach not only makes \emph{measuring} progress difficult, it completely stalls progress. Any algorithmic claims are made moot when the common basis of data is missing. We illustrate our claims by demonstrating how tightly coupled algorithmic results are to the data these algorithms use. When reflecting on these simple examples, it becomes clear that overlooking data is problematic for the field.


%The consequence of this is that accurately measuring progress across different works in the field is very challenging. First, in Section \ref{sec:summary-stats}, we set out to demonstrate the significant impact that dataset properties given by simple summary statistics such as the mean and standard deviation of episode returns can have on experimental outcomes. We present our findings in the context of the apparent disregard for the reporting of these properties by works in the field (see table \ref{tab:datasets}). In section \ref{sec:distributions} we attempt to highlight that while summary statistics may be important, they are not necessarily sufficient to properly interpret offline MARL experiments. We use the result to emphasise the utility of visualising the distribution of episode returns in a dataset, a step which is currently widely overlooked by the field. Finally, in section \ref{sec:action-space} we highlight the limits of using the distribution of episode returns as a measure of the diversity of a dataset. Instead, we propose an extension of an idea first proposed by \citet{schweighofer2022dataset} in the single-agent setting called, State-Action Coverage (SACo). We extended SACo to the multi-agent setting by computing a decentralised observation-action coverage (DecOACo) score for each agent independently, as well as state and joint-observation coverage scores.


% First, we focus on datasets in their role as control variables. We investigate the following questions: What are the most basic properties to standardise and is the field adhering to that at all? How do these properties affect performance - can they actually change algorithm preferences? If we standardised these properties, would we be able to standardise across different datasets? Are there other properties common to similarly-labelled datasets by which we could justify the standardisation of different datasets?

% Our findings show that a) the field does not standardise basic properties of datasets b) these same properties when varied can produce significantly different performance for the same algorithm c) even if we did standardise these properties, performance of the same algorithm can differ significantly on two different datasets and d) if a set of fully descriptive properties of a dataset exists, it is not clear what that set might be.

% In section \ref{sec:lit-review}, we noted that neither environment version, nor episode return mean nor episode return standard deviation are standardised across the datasets available in the offline MARL field. We now demonstrate that differences in these characteristics of a dataset can significantly affect the results produced using that dataset.

% To demonstrate how dramatic the performance discrepancy can be with even a slight mismatch in environment versioning, we report in \autoref{fig:mamujoco-versions} the performance of MADDPG+CQL trained on several Multi-Agent MuJoCo datasets but in one case the algorithm was evaluated with MuJoCo version 2.0 and another with MuJoCo 2.1. Since the dataset was generated using MuJoCo 2.1, it makes sense that the algorithm performed best when evaluated with the same version. Evaluating under version 2.0 (only one minor release version difference) caused significantly worse final performance. %The second accessibility challenge is that some works do not share download information for their datasets, or share links that are broken. Furthermore, information on how to use the datasets is usually scarce. 

% Others had similar versioning issues online\footnote{\url{https://github.com/ling-pan/OMAR/issues/3}}.

% \begin{figure}[hbtp]
%     \centering
%     \includegraphics[width=0.8\textwidth]{figures/datasets/mamujoco_versions.pdf}
%     \caption{In order to demonstrate that a minor mismatch between dataset and evaluation environment versioning can result in large performance discrepancies, we compared the performance of MADDPG+CQL on MAMuJoCo using Mujoco version 2.0 in one case and MuJoCo version 2.1 in another. The dataset was generated using MuJoCo version 2.1. We aggregated our results across datasets from three scenarios: \texttt{2 Agent HalfCheetah}, \texttt{2 Agent Ant} and \texttt{4 Agent Ant}. We also repeated each experiment across 10 random seeds. To aggregate across scenarios, we first normalised the results.}
%     \label{fig:mamujoco-versions}
% \end{figure}

\subsection{Episode return summary statistics} \label{sec:summary-stats}
In the single-agent offline RL literature, it is very common to use the summary statistics, mean and standard deviation of the episode returns, to characterise a dataset. Datasets with a higher mean episode return are often given labels such as \emph{Good} or \emph{Expert}. Similarly, the standard deviation of episode returns is commonly used as a proxy for dataset diversity, and datasets with large standard deviations are often labelled as "Mixed". Despite being widely reported in the single-agent literature, table \ref{tab:datasets} highlights how commonly offline MARL works fail to report these two statistics. In section \ref{sec:mean} and \ref{sec:std} we test the effect that the mean and standard deviation have on experimental outcomes respectively. We believe that these experiments are valuable because at present the field seems to be taking their effects for granted (and is hence commonly omitted in papers).

\subsubsection{Mean} \label{sec:mean}
To test the effect that the mean episode return has on offline MARL experiments we construct datasets with different means on three different SMAC \citep{} scenarios. For each dataset we keep the standard deviation fixed at 2 and the number of episodes fixed to 2000. For both the mean and standard deviation there is a small margin of error (see table \ref{}) since we construct the datasets by sub-sampling episodes from OG-MARL datasets \citep{formanek2023ogmarl}.  We then train two offline MARL algorithms on each dataset respectively and report the final evaluation episode return. We repeat the experiment across 10 random seeds. We then aggregated all results across scenarios, algorithms and seeds using bootstrap confidence intervals \citep{agarwal2021deep,gorsane2022emarl}. 

\begin{figure}[hbtp]
    \centering
    \begin{tabular}{c}
        \begin{subfigure}[p]{0.35\textwidth}
            \centering
            \scriptsize
            \setstretch{1.5}
                \begin{tabular}{c|c}
                & $\mu$ \\\hline
                \dotred & $7\pm0.1$  \\
                \dotgreen & $10\pm0.1$  \\
                \dotorange & $13\pm0.1$  \\
                \dotblue & $16\pm0.1$  \\
                \bottomrule
                \end{tabular}
        \caption{Mean episode return for each class of dataset. Datasets were generated for three SMAC scenarios \texttt{5m\_vs\_6m}, \texttt{3s5z\_vs\_3s6z} and \texttt{2s3z}.}
        \label{fig:mean-matters-means}
        \vspace{1em}
      \end{subfigure}\\
      \end{tabular}
    \hspace{1em}
    \begin{subfigure}[p]{0.55\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/datasets/mean_matters.pdf}
         \caption{Results comparing the final performance of offline MARL algorithms trained on datasets with different mean episode returns. Results are aggregated using bootstrap confidence intervals \citep{agarwal2021deep}. To facilitate aggregation across different scenarios and algorithms, results are first normalised.}
         \label{fig:mean-matters-results}
    \end{subfigure}
      \caption{To demonstrate the effect that the mean episode return of a dataset has on the final performance of an offline MARL algorithm, we generated four datasets with mean episode returns given in \autoref{fig:mean-matters-means}. We then train an offline MARL algorithm for 50k training steps on each of the datasets and compare the final performance of the algorithm across the different datasets. Finally, we repeated the experiment across three different SMAC scenarios, two different algorithms and 10 random seeds. The aggregated results are given in \autoref{fig:mean-matters-results}.}
\label{fig:mean-matters}
\end{figure}

Figure \ref{fig:mean-matters} illustrates that the mean episode return of the dataset is positively correlated with the final performance of the two algorithms we tested. While this may seem obvious, it is clear that without knowing the mean episode return of a dataset used in one paper, it would be very challenging to know how to compare the result to another work that used a different dataset with a different mean. Comparing the final performance of an offline RL algorithm to the mean episode return of the dataset is common practice in the single-agent literature~\citep{gulcehre2020rl, agarwal2019optimistic}, but currently, very few offline MARL researchers are doing it.

\subsubsection{Standard deviation} \label{sec:std}

Arguably one of the most important properties of a dataset in offline RL is experience diversity \citep{agarwal2019optimistic}. In the single-agent setting, it is well-understood that many offline RL algorithms benefit from more diverse datasets~\citep{schweighofer2022dataset}. It is usually beneficial because diverse experience leads to better coverage of the state and action spaces, resulting in fewer out-of-distribution (OOD) actions, which are known to cause issues when training offline~\citep{fujimoto2019bcq}. However, we believe that the effect of diversity in the offline MARL setting is less well understood and should not be naively taken for granted given the knowledge from the single-agent setting. Work by \citet{pjap}, studying two-player polynomial games, points to there being a more complex relationship between dataset diversity and final performance in the offline MARL setting than might have been assumed by the community. To test the effect that the standard deviation has on the outcome of an offline MARL experiment in practice, we generate several datasets in SMAC with varying standard deviations, similar to the previous section for the mean. Once again, we repeat the experiment across three scenarios, two algorithms and ten random seeds.

\begin{figure}[hbtp]
    \centering
    \begin{subfigure}[p]{0.47\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/datasets/std_matters_hist.pdf}
         \caption{Histograms of the episode returns of five datasets with differing standard deviations but the same mean are given.}
         \label{fig:std_matters_violins}
    \end{subfigure}
    \hspace{1em}
    \begin{tabular}{c}
        \begin{subfigure}[p]{0.46\textwidth}
            \centering
            \scriptsize
            \setstretch{1.5}
                \begin{tabular}{c|cc}
                 & $\mu$ & $\sigma^2$ \\\hline
                \dotblue & $10\pm0.1$ & $0.5\pm0.02$ \\
                \dotorange & $10\pm0.1$ & $1.0\pm0.1$ \\
                \dotgreen & $10\pm0.1$ & $2.0\pm0.1$ \\
                \dotred & $10\pm0.1$ & $4.0\pm0.1$ \\
                \dotpurple & $10\pm0.1$ & $6.0\pm0.1$ \\
                \bottomrule
                \end{tabular}
        \caption{Dataset mean and standard deviation.}
        \vspace{1em}
      \end{subfigure}\\
    %\noalign{\bigskip}%
      \begin{subfigure}[p]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/datasets/std_matters_results.pdf}
         \caption{The aggregated results across scenarios, algorithms and random seeds are given for each dataset. The median, interquartile mean and mean are all given with bootstrap confidence intervals \citep{agarwal2021deep}.}
         \label{fig:std_matters}
      \end{subfigure}
      \end{tabular}
      \caption{To demonstrate the surprising effect that the standard deviation (std) can have on the performance of an offline MARL experiment we generated 5 datasets that each had the same mean but differing std. We then trained an algorithm on the data and reported the final performance. We repeated the experiment across three different SMAC scenarios, 2 two different algorithms and 10 random seeds. We then aggregated the results as per \cite{gorsane2022emarl}.}
\end{figure}

In \autoref{fig:std_matters}, we see that the performance of the offline MARL algorithms is not optimal with either a very large or a very small standard deviation. Instead, algorithms performed the best when the episode return's standard deviation was somewhere in the middle. This surprising result (from the perspective of a single-agent offline RL researcher) reinforces our argument that papers in offline MARL should report the standard deviation of the episode return in their datasets precisely because our understanding of its effect is not widely understood. Furthermore, it highlights that there is still plenty of research to be done to explore how the quality and diversity of multi-agent data affect the final performance of offline MARL algorithms.

\subsection{Episode return distribution} \label{sec:distributions}

Having demonstrated the significant and surprising effect that datasets with different means and standard deviations can have on offline MARL experiments, we now test whether these properties are sufficient to describe experimental datasets. To test this, we generated two datasets on the 2x3 HalfCheetah environment in Multi-Agent MuJoCo \citep{}, such that they had visibly different episode return distributions (as can be seen from the histograms in figure \ref{fig:std_and_mean_hist}) but with similar mean and standard deviations (see table \ref{tab:same-summary-stats}). We are reminded of the famous Anscombe's quartet. We then trained the offline MARL algorithm MADDPG+CQL \citep{baselines_paper} on the two datasets and repeated the experiment across 10 random seeds.

\begin{figure}[hbtp]
    \centering
     \begin{subfigure}[p]{0.46\textwidth}
         \centering
         \includegraphics[width=\textwidth]{figures/datasets/std_and_mean_hist.pdf}
         \caption{Histogram of the episode returns in either dataset.}
         \label{fig:std_and_mean_hist}
    \end{subfigure}
    \hspace{1em}
    \begin{tabular}{c}
    \begin{subfigure}[p]{0.46\textwidth}
         \centering
         \scriptsize
         \setstretch{1.5}
         \begin{tabular}{c|cc}
                 & $\mu$ & $\sigma^2$ \\\hline
                \dotorange & $3688$ & $2885$ \\
                \dotblue & $3665$ & $2866$ \\
                \bottomrule
        \end{tabular} \label{tab:same-summary-stats}
        \caption{Mean and standard deviation of either dataset.}
        \vspace{1em}
      \end{subfigure}\\
    \begin{subfigure}[p]{0.45\textwidth}
        \centering
         \includegraphics[width=\textwidth]{figures/datasets/std_and_mean_results_halfcheetah.pdf}
         \caption{The aggregated results across ten random seeds for each dataset. The median, interquartile mean and mean are all given with bootstrap confidence intervals \citep{agarwal2021deep}.}
         \label{fig:mean_std_not_enough}
     \end{subfigure} \label{tab:same-summary-stats}
    \end{tabular}
     \caption{We generated two datasets on 2-Agent Halfcheetah each with very similar episode return means and standard deviations, but distinct data distributions. We then trained MADDPG+CQL on each dataset and reported its final performance after 50,000 training steps. We repeated the experiment over 10 random seeds.}
\end{figure}

In figure \ref{fig:mean_std_not_enough} we can see that the final performance of MADDPG+CQL when trained on the two datasets with very similar summary statistics was significantly different. This result corroborates our claim that while summary statistics are essential for understanding offline MARL datasets, they are not enough. Visualising the dataset distribution is also an essential step, which no one in the multi-agent field is adopting, in contrast to the single-agent field \citep{}. While visualising the distribution of episode returns can be achieved with a histogram, we argue that violin plots are also a good choice and come with several advantages. Most notable of which is that unlike histograms which require careful tuning of the number and size of buckets, violin plots automatically plot a continuous approximation of the distribution, making it easier to use.

\subsection{Multi-agent action coverage} \label{sec:action-space}

We previously showed that datasets with standardised mean and standard deviation of episode returns can still produce significantly different performance. We argued that visualising the distribution of episode returns helps to explain the difference in performance. We now further test whether the mean, standard deviation and distribution of episode returns in a dataset is sufficient to describe the dataset - in other words, can a dataset be fully described by its episode returns?

We access datasets from \citet{formanek2023ogmarl} and \citet{cfcql} on the $5m\_vs\_6m$ SMAC task in order to answer this question. In particular, the "Good", "Medium" and "Poor" datasets from \citet{formanek2023ogmarl} are compared to the "Medium-Replay", "Medium" and "Expert" datasets from \citet{cfcql}, respectively, since they have similar means and standard deviations. We uniformly subsample the original datasets to a standard size of within an episode of $120~000$ transitions. We then report the subsampled datasets' means, standard deviations and distributions of episode returns in Figure {ref}.


\begin{figure}[hbtp]
    \centering
    \begin{subfigure}[p]{0.45\textwidth}
    \resizebox{6cm}{!}{
        \begin{tabular}{lcc}
        \hline
            Dataset & Mean & Standard deviation \\
            \hline
            OG-MARL: & & \\
            Good & 16.61 & 4.68 \\
            Medium & 12.64 & 5.06 \\
            Poor & 7.46 & 1.48 \\
            CFCQL: & & \\
            Expert & 18.17 & 3.79 \\
            Medium & 12.04 & 4.36 \\
            Medium-Replay & 9.02 & 2.59 \\
            \hline
            \hline
        \end{tabular}
        }
        \caption{Means and standard deviations of the episode returns in subsampled datasets.}
        \label{tab:dataset_sizes}
    \end{subfigure}
    \hfill
    \begin{subfigure}[p]{0.45\textwidth}
        \includegraphics[width=1\linewidth]{figures/saco_and_oaco/violin_5m_vs_6m_120000.vlt.pdf}
        \caption{The violin plots of considered datasets.}
        \label{fig:violins}
    \end{subfigure}
\label{fig:describe_5m_vs_6m}
\end{figure}


We trained the offline MARL algorithm IDRQN + CQL on the subsampled datasets and repeated the experiment across 10 random seeds. The results are illustrated by Figure (ref).


\begin{table}[hbtp]
    \centering
    \begin{tabular}{ccc}
         \hline
         Dataset & Return & StdErr \\
         \hline
         Good & 16.19 & 1.64 \\
         Expert & 17.03 & 0.97 \\
         \hline
         Medium (OG-MARL) & 15.79 & 2.93 \\
         Medium (CFCQL) & 11.42 & 0.86 \\
         \hline
         Poor & 10.87 & 2.63 \\
         Medium-Replay & 10.29 & 1.19 \\
         \hline
         \bottomrule
    \end{tabular}
    \caption{Temp}
    \label{tab:temp}
\end{table}

Observe that the results using the "Medium" dataset from \citet{cfcql} are significantly worse than those using the "Medium" dataset from \citet{formanek2023ogmarl}. This difference is unexplained by the episode return descriptors of the datasets, since the datasets have similar summary statistics and the distributions of their episode returns also appear quite similar.

Clearly, there are other significant differences between the datasets which escape the reach of our current descriptors. Note all of our current descriptors are based on episode return, which is itself a summary of a trajectory and so is a level removed from the actual contents of the dataset. \citet{schweighofer2022dataset} showed that their proposed measure of dataset diversity, State-Action Coverage (SACo), has a significant effect on offline RL experiments. We extend the definition of SACo to the multi-agent setting.

\textbf{Joint SACo.} Joint SACo is defined in the same way as SACo - as the ratio between the number of unique state-action pairs and the total number of state-action pairs in a dataset - with the only difference being that the action in this case refers to the joint action of all agents in the system.

The Joint SACo values of the $5m\_vs\_6m$ datasets are illustrated by Table \ref{tab:saco}. 

\begin{table}[hbtp]
    \centering
    \begin{tabular}{lc}
         \hline
         Dataset & Joint SACo \\
         \hline
         Good & 0.85 \\
         Expert & 0.13 \\
         \hline
         Medium (OG-MARL) & 0.89 \\
         Medium (CFCQL) & 0.11 \\
         \hline
         Poor & 0.88 \\
         Medium-Replay & 0.96\\
         \hline
         \bottomrule
    \end{tabular}
    \caption{Joint SACo}
    \label{tab:saco}
\end{table}

The datasets from \citet{cfcql} which do not contain replay data have low Joint SACo values of $13\%$ and $11\%$, meaning that the overwhelming majority of these datasets are repetitions of previously seen state-action pairs. The "Medium-Replay" dataset, however, has the highest Joint SACo value of all the datasets, $96\%$, and is 

About $89$ percent of the "Medium" dataset from \citet{cfcql} is repetitions of previously-seen state-action pairs. When we compare that to 11 percent repeated content in the "Medium" dataset from \citet{formanek2023ogmarl}, it may explain the difference in performance in Figure (ref). 

However, if there is a correlation it may not be generalised, since there is not a large difference in performance generated by the "Good" dataset and "Expert" dataset, and their coverage measures show that the "Expert" dataset has far less diverse experience than the "Good" dataset.

One potential explanation is that in the given setting (i.e. training with IDRQN + CQL on a SMAC dataset) datasets with high episode returns produce results which are more robust to low coverage. This hypothesis is strengthened by the fact that in the results reported by \cite{schweighofer2022dataset}, CQL trained on the "Expert"-type datasets with high Trajectory Quality (TQ) \citep{schweighofer2022dataset} performs well across varying coverage levels. Further investigation is required, since we have observed in subsection \ref{sec:std} that dataset diversity does not always have the same effect in offline MARL as in single agent offline RL.

Our understanding of the composition of SMAC datasets has been lacking thus far, which is concerning because SMAC is the most popular environment for offline datasets for research in MARL. We have found that datasets generated by rolling out a frozen policy run the risk of having low diversity, which may in turn have significant and unpredictable effects on experiment outcomes.


\textbf{Takeaways}

All of our findings point towards each unique dataset being exactly that - unique. Although we observed some trends in algorithm performance when varying dataset summary statistics, some of those trends were surprising and can absolutely not be assumed to have a simple general form for all dataset-algorithm combinations. We therefore stress that a) assumptions from single-agent offline RL can not be transplanted into offline MARL and b) while it is important to test offline algorithms on a variety of datasets, it is not clear what variety means in the offline context, nor which axis of property variation in a dataset will provide adequate coverage of the desired problem space for offline MARL.

 The first steps towards producing adequate coverage of the desired problem space for offline MARL is to be able to measure such coverage. We defined three measures for dataset coverage for offline MARL, and showed how insights can be obtained using these measures. Although further research is required, we have already found insights using these measures which have previously not been accessible to the field.

==> tables/baseline_envs.tex <==
\begin{table}[h]
\centering
\scriptsize
\setstretch{1.5}
\caption{({\cmark \, present}, {\xmark \, absent})} \label{tab:baseline_envs}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c}
& \texttt{2s3z} & \texttt{3s v 5z} & \texttt{5m v 6m} & \texttt{6h v 8z} & \texttt{MMM} & \texttt{10m v 11m} & \texttt{3s v 3z} & \texttt{3s5z} & \texttt{1c3s5z} & \texttt{2c v 64zg} & \texttt{3s5z v 3s6z} & \texttt{corridor} \\ \hline
 MAICQ & \cmark & \xmark & \xmark & \xmark & \cmark & \cmark & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark \\
 MADT & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \cmark & \xmark & \xmark & \cmark & \cmark \\
 OMAR & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \cmark & \cmark & \cmark & \xmark & \xmark \\
 CFCQL & \cmark & \cmark & \cmark & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark \\
 OMAC & \xmark & \xmark & \cmark & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \cmark & \cmark \\
 OMIGA & \xmark & \xmark & \cmark & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \cmark & \xmark & \cmark \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}

==> tables/dataset_sizes.tex <==
\begin{table}[hbtp]
    \centering
    \begin{tabular}{ccc}
    \hline
        Dataset & Total size & Subsampled size \\
        \hline
        OG-MARL: Good & 996726 & 24994 \\
        OG-MARL: Medium & 996855 & 24998 \\
        OG-MARL: Poor & 934504 & 24991 \\
        OMIGA: Good & 27733 & 24979 \\
        OMIGA: Medium & 27716 & 24983 \\
        OMIGA: Poor & 22746 & 22746 \\
        CFCQL: Expert & 128535 & 24998 \\
        CFCQL: Medium & 135255 & 24990 \\
        CFCQL: Medium-Replay & 118404 & 24972 \\
        CFCQL: Mixed & 131702 & 24979 \\
        \hline
        \hline
    \end{tabular}
    \caption{Dataset sizes for $5m\_vs\_6m$}
    \label{tab:dataset_sizes}
\end{table}

==> tables/macql.tex <==
\begin{table}[htbp]
\centering
\scriptsize
\setstretch{1.5}
\caption{}\label{tab:macql}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{c|c|c|c}
\textbf{Paper} & \textbf{Nomenclature} & \textbf{Details Provided} & \textbf{Full Code Given?} \\

\hline 
MAICQ
% &mujocomujoco
% \begin{tabular}{c} 
% \symboldiscrete \\
% \symbolcontinuous
% \end{tabular}
& MA-CQL
 & \begin{tabular}{c} 
Loss function, value-decomposition structure
\end{tabular} &
\textcolor{xmarkcolour}{No (only single-agent CQL)}
\\
\hline 
MADT
% &
% \begin{tabular}{c} 
% \symboldiscrete \\
% \symbolcontinuous
% \end{tabular}
& CQL-MA
 & \begin{tabular}{c} 
CQL + `mixing network'
\end{tabular} & \textcolor{xmarkcolour}{No} \\

\hline
OMAR
% &
% \begin{tabular}{c}
% \symboldiscrete \\
% \symbolcontinuous
% \end{tabular}
& MA-CQL
 & \begin{tabular}{c} 
MADDPG~\citep{lowe2017maddpg}\\(Discrete: + Gumbel Softmax~\citep{jang2016categorical})
\end{tabular} &
\begin{tabular}{c} 
    \textcolor{xmarkcolour}{No (single-agent CQL,}\\
    \textcolor{xmarkcolour}{\& MADDPG without CQL)}
\end{tabular}
\\

\hline
CFCQL
% &
% \begin{tabular}{c} 
% \symboldiscrete \\
% \symbolcontinuous
% \end{tabular}
& MACQL
& \begin{tabular}{c} 
`Naive extension of CQL to multi-agent settings` + Loss function
\end{tabular} & Yes \\

\hline
OMAC
% &
% \begin{tabular}{c} 
% \symboldiscrete \\
% \symbolcontinuous
% \end{tabular}
& TODO
& \begin{tabular}{c} 
TODO
\end{tabular} & \textcolor{xmarkcolour}{TODO} \\

\hline
OMIGA
% &
% \begin{tabular}{c} 
% \symboldiscrete \\
% \symbolcontinuous
% \end{tabular}
& CQL-MA
& \begin{tabular}{c} 
Value decomposition structure + policy constraint
\end{tabular} & \textcolor{xmarkcolour}{No} \\

\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}


==> tables/map_to_vault.tex <==
\begin{landscape}
\begin{table}[p]
\centering
\scriptsize
\setstretch{1.5}
\caption{Mapping of existing datasets into the Vault format~\citep{flashbax}. \emph{Environment sources:} MAMuJoCo~\citep{peng2021facmac}, SMACv1~\citep{samvelyan2019smac}, SMACv2~\citep{ellis2022smacv2}, MPE~\citep{lowe2017maddpg}, RWARE~\citep{christianos2020SharedExperience}}\label{tab:vault_links}
\vspace{1em}
\begin{adjustbox}{max width=\linewidth}
\begin{tabular}{lllllll}

Variable in Vault & \cite{omar} MAMuJoCo & \cite{omar} MPE & \cite{cfcql} SMACv1 & \cite{omiga} SMACv1 & \cite{omiga} MAMuJoCo & \cite{alberdice} RWARE \\ \hline
 \texttt{actions} & \texttt{actions} & \texttt{actions} & \texttt{actions} & \texttt{actions} &  \texttt{actions} & \texttt{actions} \\
 \texttt{infos["legals"]} & \texttt{infos["legals"]}& \texttt{infos["legals"]}& \texttt{infos["legals"]}& \texttt{infos["legals"]}& \texttt{infos["legals"]}& \texttt{infos["legals"]} \\
 \texttt{infos["state"]} & \texttt{infos["state"]}& \texttt{infos["state"]}& \texttt{infos["state"]}& \texttt{infos["state"]}& \texttt{infos["state"]}& \texttt{infos["state"]} \\
 \texttt{observations} & \texttt{observations}& \texttt{observations}& \texttt{observations}& \texttt{observations}& \texttt{observations}& \texttt{observations} \\
 \texttt{rewards}  & \texttt{rewards} & \texttt{rewards} & \texttt{rewards} & \texttt{rewards} & \texttt{rewards} & \texttt{rewards} \\
 \texttt{terminals}  & \texttt{terminals} & \texttt{terminals} & \texttt{terminals} & \texttt{terminals} & \texttt{terminals} & \texttt{terminals} \\
  \texttt{truncations}  & \texttt{truncations}  & \texttt{truncations}  & \texttt{truncations}  & \texttt{truncations}  & \texttt{truncations}  & \texttt{truncations} \\
Does not appear & & & & & & \\
in the Vault &&&&&& \\
\hline
\end{tabular}
\end{adjustbox}
\end{table}
\end{landscape}

==> tables/num_scenarios.tex <==
\begin{table}[h]
\centering
\scriptsize
\setstretch{1.5}
\caption{Number of scenarios tested in the papers from the case study.}
\begin{adjustbox}{max width=0.9\textwidth}
\begin{tabular}{c|c|c|c|c}
      & SMAC & MAMuJoCo & MPE & Other \\ \hline
MAICQ & 4  & --        & --   & --     \\
MADT  & 21  & --        & --   & --     \\
OMAR  & 4     & 1        & 3   & --     \\
CFCQL & 4     & 1        & 3   & --     \\
OMAC  & 4     & --        & --   & --     \\
OMIGA & 4     &  3         & --   & --     \\
\bottomrule
\end{tabular}
\label{tab:scenarios}
\end{adjustbox}
\end{table}


==> tables/performance_report_stats.tex <==
\begin{table}[h]
\centering
\scriptsize
\setstretch{1.5}
\caption{Table showing the performance reporting only for the experiments making State-Of-The-Art claims about Multi-Agent Offline RL}\label{tab:perform_report}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{c|c|c|c|c}
\textbf{Paper} & \textbf{Evaluation frequency} & \textbf{Performance metrics} & \textbf{Reported statistics}  & \textbf{Seeds} \\

\hline 
MAICQ % done
& $10$ episodes per $50$ training episodes
 & \begin{tabular}{c} 
Episode return
\end{tabular} &
Mean, standard deviation - plots &
$5$
\\

\hline 
MADT %done
& \begin{tabular}{c} 
$32$ evaluation epochs at points during training    
\end{tabular} 
 & \begin{tabular}{c}
 Episode return 
\end{tabular} & Mean, standard deviation - plots & Not reported \\

\hline
OMAR
 & \begin{tabular}{c} 
Not reported
\end{tabular} &
\begin{tabular}{c} 
    Normalised score
\end{tabular} &
Mean, standard deviation - plots
& 5
\\

\hline
CFCQL
& Not reported
& \begin{tabular}{c} 
Episode return, normalised score
\end{tabular} & Mean, standard deviation - values only & 5 \\

\hline
OMAC %done
& 32 evaluation episodes at points during training
& \begin{tabular}{c} 
Episode return \\ 
Sample efficiency
\end{tabular}
& Mean, standard deviation - plots
& 5
\\

\hline
OMIGA
& $32$ episodes, sourcing method not reported
& \begin{tabular}{c} 
Episode return
\end{tabular} & Mean, standard deviation - values only & 5 \\

\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}

==> tables/related_work.tex <==
\begin{table}[H]
\centering
\scriptsize
\caption{Works in RL and an overview of their dataset, data-preprocessing and algorithmic contributions specific to the offline MARL field.} \label{tab:relateds}
\vspace{1em}
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{ cccc }
\hline
Paper & Dataset generation and use as a control variable & Dataset manipulation as an algorithmic component & Data-agnostic algorithm innovation\\
\hline
\citet{zhang2021finitesample} & .. & .. & Networked agents \\
\citet{jiang2021marldecentralised} & Self-generated and made from D4RL  & .. & Objective function improvements\\ %- a prescribed way to do MABCQ\\
\citet{maicq} & Self-generated  & .. & Objective function improvements\\%ICQ (single and multi-agent)\\
\citet{omar} & Self-generated  & Additional data sampling mechanism & Objective function improvements\\
\citet{madt} & Self-generated  & .. & Multi-agent decision transformer architecture\\
\citet{tseng2022knowledgedistill} & Self-generated  & .. & Transformer architecture with knowledge distillation\\
%\citet{formanek2023ogmarl} & Datasets as a main offering & .. & .. \\
\citet{barde2023modelbased} & Self-generated and made from D4RL & Synthesise data from a learnt world model & Supportive algorithm design\\
\citet{tian2023goodtrajectories} & Self-generated & Individual-trajectory-based dataset reconstruction & Supportive algorithm design\\
\citet{cfcql} & Self-generated and from \citet{omar} & .. & Objective function improvements\\
\citet{OMAC} & From \citet{madt} & .. & Objective function improvements\\
\citet{omiga} & Self-generated and from \citet{madt} & .. & Algorithmic improvements\\
\hline
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table} %\label{tab:relateds}


==> tables/stats_subsampled_5m_vs_6m.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{lcccc}
        \hline
            Dataset & Total size & Subsampled & Mean & Stddev \\
            \hline
            OG-MARL: & & \\
            Good & 996726 & 19991 & 16.50 & 4.75 \\
            Medium & 996855 & 19992 & 12.57 & 5.08 \\
            Poor & 934504 & 19991 & 7.43 & 1.55 \\
            OMIGA: & & \\
            Good & 27733 & 19977 & 20.00 & 1.12e-06 \\
            Medium & 27716 & 19979 & 11.02 & 0.58 \\
            Poor & 22746 & 19991 & 8.51 & 1.21 \\
            CFCQL: & & \\
            Expert & 128535 & 19992 & 18.34 & 3.64 \\
            Medium & 135255 & 19983 & 11.88 & 4.28 \\
            Medium-Replay & 118404 & 19978 & 8.95 & 2.40 \\
            Mixed & 131702 & 19978 & 15.16 & 5.06 \\
            \hline
            \hline
    \end{tabular}
    \caption{Basic information on datasets subsampled from those available.}
    \label{tab:dataset_sizes}
\end{table}


        
